Dual-space Hierarchical Learning for Goal-guided Conversational Recommendation

Proactively and naturally guiding the dialog from the non-recommendation context (e.g., Chit-chat) to the recommendation scenario (e.g., Music) is crucial for the Conversational Recommender System (CRS). Prior studies mainly focus on planning the next dialog goal~(e.g., chat on a movie star) conditioned on the previous dialog. However, we find the dialog goals can be simultaneously observed at different levels, which can be utilized to improve CRS. In this paper, we propose Dual-space Hierarchical Learning (DHL) to leverage multi-level goal sequences and their hierarchical relationships for conversational recommendation. Specifically, we exploit multi-level goal sequences from both the representation space and the optimization space. In the representation space, we propose the hierarchical representation learning where a cross attention module derives mutually enhanced multi-level goal representations. In the optimization space, we devise the hierarchical weight learning to reweight lower-level goal sequences, and introduce bi-level optimization for stable update. Additionally, we propose a soft labeling strategy to guide optimization gradually. Experiments on two real-world datasets verify the effectiveness of our approach. Code and data are available here.

==> Rebuttal.tex <==
\section{Rebuttal}

\subsection{Review 1}

Overall: 

1. Motivation of cross attention: There is some semantic relationship between goal type sequence and goal entity sequence, and thus we introduce cross attention to model this relationship and derive mutually enhanced multi-level goal representations.

2. Motivation of bi-level optimization: As we have discussed in L332-L335, joint optimizing the hierarchical weights and the model parameters leads to trivial solutions where all hierarchical weights reduce to zeros. We thus introduce bi-level optimization for a stable update on the hierarchical weights.

3. Motivation of soft labeling: Soft labeling can be traced back to the image classification task where the soft labeling technique serves as a regularization. In our work, soft labeling plays a different role. We leverage the soft labeling strategy to achieve gradual guidance and enforce the prediction closer to the final goal as the conversation went on.

Strength:
The baselines are state-of-the-art methods and thus are strong enough.

Weakness:

1. Writing: Thanks for your advice! We will improve our writing.

2. Novelty and motivation: As we have discussed in L332-L335, joint optimizing the hierarchical weights and the model parameters leads to trivial solutions where all hierarchical weights reduce to zeros. This deteriorates the CRS a lot and the CRS model learns nothing. We thus introduce bi-level optimization for a stable update on the hierarchical weights. 

3. Experiments: Besides the qualitative results in Sec 4.7, we have ablation studies in Sec 4.5 to verify the effectiveness of every design component in DHL. The qualitative results in Sec 4.7 and the ablation studies in Sec 4.5 together can analyze the effectiveness of DHL.

Questions for the Authors: Thanks for pointing this out! TG-ReDial was
constructed by human annotation based on real-world user data and we will mention this in an improved version.

\subsection{Review 2}

Weakness:

1. Thanks for your question! For a certain supervised ML task, we need to consider two key points: how to extract the feature of the task and how to define the loss function, which corresponds to the representation space and the optimization space in this CRS setting respectively.

2. We have run experiments with $8$ different seeds and the experimental results are quite robust to the randomness. we will report results with a confidence level in an improved version.

\subsection{Review 3}

Reasons to reject:

Clarity:

1. Thanks for your suggestion! As we have illustrated in L171, x represents a goal. We will make the illustration clear in an improved version.

2. Thanks for your suggestion! The topic in Definition 2 can represent a goal type or a goal entity.

Approach: we follow the MGNN work [1] to use this adjacency matrix. The attention module can derive mutually enhanced multi-level goal representations and thus can be more effective than the coarse adjacency matrix modeling. To clarify your doubts, we further remove the adjacency matrix from DHL and run experiments on DuRecDial and TGReDial. The results without the adjacency matrix are a little worse than that with the adjacency matrix (DHL DuRecDail Acc from 83.51 to 82.47, Rec from 62.62 to 60.04, Prec from 72.52 to 69.37, F1 from 65.25 to 64.21, LS from 13.52 to 12.90; DHL TGReDial Acc from 39.99 to 38.58, Rec from 20.78 to 18.15, Prec from 46.32 to 42.24, F1 from 20.43 to 18.20, LS from 24.82 to 22.29).
We suppose the reason may be that cross attention can better capture this information with the help of the cooccurrence information.

We will add the above discussion in an improved version.

[1] Zeming Liu, Ding Zhou, Hao Liu, Haifeng Wang, Zheng-Yu Niu, Hua Wu, Wanxiang Che, Ting Liu, and Hui Xiong. 2022. Graph-grounded goal planning for conversational recommendation. IEEE Transactions on Knowledge and Data Engineering.

\subsection{Review 4}

Weaknesses:

1. Thanks for your suggestion! The recommendation goal is a goal in the goal sequence. As we have discussed in L184-L193 Problem Statement, we aim to simultaneously plan goal sequences (goal prediction) to proactively and naturally lead the conversation to reach the final recommendation goal (some goal in the goal sequence). We will illustrate this part in an improved version.

2. As we have discussed in Related work, there are two research lines in the conversational recommender system: one from the recommender system and one from the dialogue system. The first research line aims to infer the user’s interest by historical interactions and the second line aims to enforce natural semantic transitions in multi-turn human-machine natural language interactions. There are only a few works in the second research line and our work belongs to this line. We have included all closely-related work in this research line.



\subsection{General}
Many thanks for your valuable and constructive comments on clarifying, correcting, and improving the materials in this paper! We will carefully revise the paper according to your comments.



==> Sec7_limitations.tex <==
\section{Limitations}
%
The proposed DHL relies on annotated data to train the model, and thus the expensive cost of data annotation becomes one limitation of DHL.
%
Few-shot learning methods may be introduced to mitigate this issue.
%One limitation of DHL is the lack of data annotation.
%Lack of data annotation.
%
Another limitation is the hand designed topic threads are not enough to reflect the changing user dynamics. 
%
A possible direction is to directly generate topic threads from the previous collected data by using advanced NLP techniques.
%
We leave these to future work.
%Hands designed topic thread may not capture the changing user dynamics.

==> Sec8_ethics.tex <==
%\section{Ethics}
